Microvariability in BL Lac: Zooming into the Innermost Blazar Regions

In this work, we present the results of our multi-band microvariability study of the famous blazar BL Lac. We performed microvariablity observations of the source in the optical VRI bands for 4 nights in the year 2016. We studied the intranight flux and spectral variability of the source in detail with an objective to characterize microvariability in the blazars, a frequently observed phenomenon in blazars. The results show that the source often displays a fast flux variability with an amplitude as large as ~ 0.2 magnitude within a few hours, and that the color variability in the similar time scales can be characterized as "bluer-when-brighter" trend. We also observed markedly curved optical spectrum during one of the nights. Furthermore, the correlation between multi-band emission shows that in general the emission in all the bands are highly correlated; and in one of the nights V band emission was found to lead the I band emission by ~ 20 minutes. The search for characteristic timescale using auto-correlation function and the structure function analyses reveals characteristic timescale of ~ 48 minutes in one of the R band observations. We try to explain the observed results in the context of the passage of shock waves through the relativistic outflows in blazars.

==> citations.tex <==
 \bibitem{Meier12} Meier, D.~L.\ ,
 Black Hole Astrophysics: The Engine Paradigm, Springer, Verlag Berlin Heidelberg, 
{\bf 2012}

\bibitem{Bhatta2017} 
 Bhatta, G.,\
 Radio and $\gamma$-Ray Variability in the BL Lac PKS  $0219-164$: Detection of Quasi-periodic Oscillations in the Radio Light Curve,  {\em ApJ}, {\bf 2017}, 487, 7B

 \bibitem{Bhatta2016b}  
 Bhatta, G., Zola S., Stawarz, L., et al.\ 
Detection of Possible Quasi-periodic Oscillations in the Long-term Optical Light Curve of the BL Lac Object OJ 287, 
{\em ApJ}, {\bf 2016}, 832, 47


\bibitem{Zola2016} Zola, S., Valtonen, M., Bhatta, G., et al.\
A Search for QPOs in the Blazar OJ287: Preliminary Results from the 2015/2016 Observing Campaign
{\em Galaxies}, {\bf 2016}, 4, 41

\bibitem{MG85}
Marscher, A.~P., \& Gear, W.~K.\
{Models for high-frequency radio outbursts in extragalactic sources, with application to the early 1983 millimeter-to-infrared flare of 3C 273}.  {\em ApJ} {\bf 1985}, 298, 114 

\bibitem{Camenzind92} 
{The lighthouse effect of relativistic jets in blazars - A geometric origin of intraday variability}
Camenzind, M., \& Krockenberger, M.\ {\em A\&A} {\bf 1992}, 255, 59 

\bibitem{Wagner95}
Wagner, S.~J., \& Witzel, A.
{Intraday Variability In Quasars and BL Lac Objects}, {\em ARAA} {\bf 1995},  33, 163

\bibitem{bhatta013}
{Bhatta G., Webb J. R, and Hollingsworth H. et al.} The 72-h WEBT microvariability observation of blazar S5 0716 + 714 in 2009. {\em A\&A} {\bf 2008}, 558, A92.

\bibitem{Quirrenbach1992} Quirrenbach, A., Witzel, A., Kirchbaum, T.~P., et al.\ 
Statistics of intraday variability in extragalactic radio sources
{\bf 1992}, {\em A\&A},  258, 279

\bibitem{Heidt1996} Heidt, J., \& Wagner, S.~J.\ 
Statistics of optical intraday variability in a complete sample of radio-selected BL Lacertae objects,
{\bf 1996}, {\em A\&A},  305, 42

\bibitem{Bai1998} Bai, J.~M., Xie, G.~Z., Li, K.~H., Zhang, X., \& Liu, W.~W.\ 
The intraday variability in the radio-selected and X-ray-selected BL Lacertae objects
{\bf 1998}, {\em A\&AS},  132, 83

\bibitem{Kraus2003} Kraus, A., Krichbaum, T.~P., Wegner, R., et al.\  
Intraday variability in compact extragalactic radio sources. II. Observations with the Effelsberg 100 m radio telescope
{\bf 2003}, {\em A\&A}, 401, 161

\bibitem{Howard2004} Howard, E.~S., Webb, J.~R., Pollock, J.~T., \& Stencel, R.~E.\ 
Microvariability and Long-Term Variability of Four Blazars
{\bf 2004}, {\em AJ}, 127, 17

\bibitem{Rani2011} Rani, B., Gupta, A.~C., Joshi, U.~C., Ganesh, S., \& Wiita, P.~J.\ 
Optical intraday variability studies of 10 low energy peaked blazars
{\bf 2011}, {\em MNRAS}, 413, 2157

\bibitem{Gaur2012} Gaur, H., Gupta, A.~C., Strigachev, A., et al.\  
Optical flux and spectral variability of blazars
{\em MNRAS}, {\bf 2012}, 425, 3002

\bibitem{Bachev2012} Bachev, R., Semkov, E., Strigachev, A., et al.\ 
The nature of the intra-night optical variability in blazars
{\em MNRAS}, {\bf 2012}, 424, 2625

\bibitem{Guo2016} {{Guo}, Y.~C. and {Hu}, S.~M. and {Li}, Y.~T. and {Chen}, X.}
Statistical analysis of the temporal properties of BL Lacertae,
{\em MNRAS}, {\bf 2016}, 460, 1790


 %Reference 1

\bibitem{bhatta015}
Bhatta, G., et al.\
Discovery of a Highly Polarized Optical Microflare in Blazar S5 0716+714 during the 2014 WEBT Campaign. {\em ApJ} {\bf 2015} 809L, 27B

\bibitem{bhatta016}
Bhatta, G., Stawarz, L., Ostrowski, M., et al. 
Multifrequency Photo-polarimetric WEBT Observation Campaign on the Blazar S5 0716+714: Source Microvariability and Search for Characteristic Timescales 
{\em ApJ} {\bf 2016}, 831, 92B

 \bibitem{Bhatta2016a} 
 Bhatta, G.,\
Investigating the Innermost Jet Structures of Blazar S5 0716+714 Using Uniquely Dense Intra-day Photo-polarimetric Observations, 
{\em Galaxies}, {\bf 2016} 4, 56 




\bibitem{Bhatta2017b}Bhatta G., Mohorian, M., and Bilinsky, I.
Hard X-ray Properties of NuSTAR Blazars
ApJ submitted; http://arxiv.org/abs/1710.09910


\bibitem{Wehrle2016} Wehrle, A.~E., Grupe, D., Jorstad, S.~G., et al.\ 
Erratic Flaring of BL Lac in 2012-2013: Multiwavelength Observations
{\bf 2016}, {\em ApJ}, 816, 53

\bibitem{Raiteri2013} Raiteri, C.~M., Villata, M., D'Ammando, F., et al.\ 
The awakening of BL Lacertae: observations by Fermi, Swift and the GASP-WEBT
{\bf 2013}, {\em MNRAS}, 436, 1530

\bibitem{Raiteri2010} Raiteri, C.~M., Villata, M., Bruschini, L., et al.\ 
Another look at the BL Lacertae flux and spectral variability. Observations by GASP-WEBT, XMM-Newton, and Swift in 2008-2009
 {\bf 2010}, {\em A\&A}, 524, A43

\bibitem{Villata2009} Villata, M., Raiteri, C.~M., Larionov, V.~M., et al.\	
The correlated optical and radio variability of BL Lacertae. WEBT data analysis 1994-2005,
{\bf 2009}, {\em A\&A},  501, 455

\bibitem{Bottcher2003} B{\"o}ttcher, M., Marscher, A.~P., Ravasio, M., et al.\ 
Coordinated Multiwavelength Observations of BL Lacertae in 2000,
{\bf 2003}, {\em ApJ}, 596, 847


\bibitem{Speziali1998} Speziali, R., \& Natali, G.\ 
BVI microvariability in BL Lacertae during the summer 1997 outburst
{\bf 1998}, {\em A\&A},  339, 382

\bibitem{Massaro1998} Massaro, E., Nesci, R., Maesano, M., Montagni, F., \& D'Alessio, F.\ 
Fast variability of BL Lacertae at 1mum
{\bf 1998}, {\em MNRAS}, 299, 47

\bibitem{Nesci1998} Nesci, R., Maesano, M., Massaro, E., et al.\ 
Intraday variability of BL Lacertae in the great 1997 outburst
{\bf 1998}, {\em A\&A},  332, L1

\bibitem{Clements2001} Clements, S.~D., \& Carini, M.~T.\ 
Multiband Microvariability Observations of BL Lacertae during the Outburst of 1997
{\bf 2001}, {\em AJ},  121, 90

\bibitem{Zhai2012} Zhai, M., \& Wei, J.~Y.\
Intra-night optical multiband variability of BL Lacertae during the 2011 outburst
{\bf 2012}, {\em A\&A}, 538, A125

\bibitem{Agarwal2015} Agarwal, A., \& Gupta, A.~C. 
Multiband optical variability studies of BL Lacertae
{\bf 2015}, {\em MNRAS}, 450, 541

\bibitem{Gaur2015} Gaur, H., Gupta, A.~C., Bachev, R., et al.\ 
Nature of intranight optical variability of BL Lacertae
{\bf 2015}, {\em MNRAS}, 452, 4263




\bibitem{Papadakis2003} Papadakis, I.~E., Boumis, P., Samaritakis, V., \& Papamastorakis, J.\ 
Multi-band optical micro-variability observations of BL Lacertae
{\bf 2003}, {\em A\&A},  397, 565

\bibitem{Villata2004} Villata, M., Raiteri, C.~M., Aller, H.~D., et al.\ 
The WEBT campaigns on BL Lacertae. Time and cross-correlation analysis of optical and radio light curves 1968-2003
{\bf 2004}, {\em A\&A},  424, 497

\bibitem{Abdo2011} Abdo, A.~A., Ackermann, M., Ajello, M., et al.\ 
The First Fermi Multifrequency Campaign on BL Lacertae: Characterizing the Low-activity State of the Eponymous Blazar
{\bf 2011}, {\em ApJ}, 730, 101

\bibitem{Cohen2015} Cohen, M.~H., Meier, D.~L., Arshakian, T.~G., et al.
Studies of the Jet in Bl Lacertae. II. Superluminal Alfvén Waves
{\bf 2015}, {\em ApJ}, 803, 3


\bibitem{Marscher2008} Marscher, A.~P., Jorstad, S.~G., D'Arcangelo, F.~D., et al.\ 
The inner jet of an active galactic nucleus as revealed by a radio-to-$\gamma$-ray outburst
{\bf 2008}, {\em Nature}, 452, 966

\bibitem{Arlen2013} Arlen, T., Aune, T., Beilicke, M., et al.
Rapid TeV Gamma-Ray Flaring of BL Lacertae
{\em ApJ}, {\bf 2013} 762, 92

\bibitem{Gaur2014} Gaur, H., Gupta, A.~C., Wiita, P.~J., et al. 
Anti-correlated Optical Flux and Polarization Variability in BL Lac
 {\bf 2014}, {\em ApJL}, 781, L4

\bibitem{Webb2016} Webb, J.\ 
Multi-Frequency Blazar Micro-Variability as a Tool to Investigate Relativistic Jets
{\em Galaxies}, {\bf 2016}, 4, 15

\bibitem{Howell1988} Howell, S.~B., Warnock, A., III, \& Mitchell, K.~J.\ 
Statistical error analysis in CCD time-resolved photometry with applications to variable stars and quasars
{\bf 1988}, {\em AJ}, 95, 247

\bibitem{bessel98} Bessell, M. S., Castelli, F., \& Plez, B.\
Model atmospheres broad-band colors, bolometric corrections and temperature calibrations for O - M stars
{\em A\&A}, {\bf 1998} 333, 231

\bibitem{vau03}Vaughan, S., Edelson, R., Warwick, R. S., \& Uttley, P.
On characterizing the variability properties of X-ray light curves from active galaxies
 {\bf 2003}, {\em MNRAS}, 345, 1271

\bibitem{Aleksic2015} Aleksi{\'c}, J., Ansoldi, S., Antonelli, L.~A., et al.\ 
The 2009 multiwavelength campaign on Mrk 421: Variability and correlation studies
{\em A\&A}, {\bf 2015}, 576, A126

\bibitem{Zhang2013} Zhang, Y.-H., Bian, F.-Y., Li, J.-Z., \& Shang, R.-C.\ 
Optical observations of BL Lacertae in 2004-2005
 {\bf 2013}, {\em MNRAS}, 432, 1189

\bibitem{EK88}
 Edelson, R. A., \& Krolik, J. H.\ 
 The discrete correlation function - A new method for analyzing unevenly sampled variability data, 
{\em ApJ}, {\bf 1988} 333, 646

\bibitem{Abdo2010} Abdo, A.~A., Ackermann, M., Ajello, M., et al.\ 
Gamma-ray Light Curves and Variability of Bright Fermi-detected Blazars
 {\em ApJ}, {\bf 2010}, 722, 520 

\bibitem{Simonetti85}Simonetti J. H., Cordes J. M., Heeschen D. S.\ 
Flicker of extragalactic radio sources at two frequencies,
{\em ApJ}, {\bf 1985}, 704, L129

\bibitem{Hughes1992} Hughes, P.~A., Aller, H.~D., \& Aller, M.~F.\ 
The University of Michigan radio astronomy data base. I - Structure function analysis and the relation between BL Lacertae objects and quasi-stellar objects
{\em ApJ}, {\bf 1992}, 396, 469

%***************************************************************


\bibitem{Lainela1993} Lainela, M., \& Valtaoja, E.\ 1993,	
Structure Function Analysis of High Radio Frequency Variability in the Metsaehovi Monitoring Sample of Active Galactic Nuclei,
{\em ApJ}, {\bf 1993}, 416, 485

\bibitem{Paltani1997} Paltani, S., Courvoisier, T.~J.-L., Blecha, A., \& Bratschi, P.\ 
Very rapid optical variability of PKS 2155-304
{\em A\&A}, {\bf  1997}, 327, 539

\bibitem{Zhang02}Zhang, Y. H.
Four Years of Monitoring Blazar PKS 2155-304 with BeppoSAX: Probing the Dynamics of the Jet,
{\em ApJ}, {\bf 2002}, 572, 762

\bibitem{Emmanoulopoulos10}Emmanoulopoulos, D.; McHardy, I. M.; Uttley, P.
On the use of structure functions to study blazar variability: caveats and problems,
{\em MNRAS}, {\bf 2010}, 404, 931E

\bibitem{Narayan2012} Narayan, R., \& Piran, T.\ 
Variability in blazars: clues from PKS 2155-304
 {\bf 2012}, {\em MNRAS}, 420, 604

\bibitem{Marscher2014} Marscher, A.~P.\ 
Turbulent, Extreme Multi-zone Model for Simulating Flux and Polarization Variability in Blazars
{\em ApJ}, {\bf 2014}, 780, 87 

\bibitem{Fuhrmann2014} Fuhrmann, L., Larsson, S., Chiang, J., et al.\ 
Detection of significant cm to sub-mm band radio and $\gamma$-ray correlated variability in Fermi bright blazars
{\em MNRAS}, {\bf 2014}, 441, 1899


\bibitem{Mangalam1993} Mangalam, A.~V., \& Wiita, P.~J.\ 
Accretion disk models for optical and ultraviolet microvariability in active galactic nuclei
{\em ApJ}, {\bf 1993}, 406, 420

\bibitem{Hardee1999} Hardee, P.~E., \& Rosen, A.\ 
On the Dynamics and Structure of Three-dimensional Trans-Alfvénic Jets
{\em ApJ}, {\bf 1999}, 524, 650 

%Reference 2
\bibitem{Kirk098}
{{Kirk}, J.~G. and {Rieger}, F.~M. and {Mastichiadis}, A.} Particle acceleration and synchrotron emission in blazar jets.
{\em A\&A} {\bf 1998}, 333, 452K.
















